RoCOCO: Robustness Benchmark of MS-COCO to Stress-test Image-Text Matching Models

With the extensive use of vision-language models in various downstream tasks, evaluating their robustness is crucial. In this paper, we propose a benchmark for assessing the robustness of vision-language models. We believe that a robust model should properly understand both linguistic and visual semantics and be resilient to explicit variations. In pursuit of this goal, we create new variants of texts and images in the MS-COCO test set and re-evaluate the state-of-the-art (SOTA) models with the new data. Specifically, we alter the meaning of text by replacing a word, and generate visually altered images that maintain some visual context while introducing noticeable pixel changes through image mixing techniques.Our evaluations on the proposed benchmark reveal substantial performance degradation in many SOTA models (e.g., Image-to-Text Recall@1: 81.9\% $\rightarrow$ 48.4\% in BLIP, 66.1\% $\rightarrow$ 37.6\% in VSE$\infty$), with the models often favoring the altered texts/images over the original ones. This indicates the current vision-language models struggle with subtle changes and often fail to understand the overall context of texts and images. Based on these findings, we propose semantic contrastive loss and visual contrastive loss to learn more robust embedding. Datasets and code are available at {\url{https://github.com/pseulki/rococo}}.

==> figures/influence_of_word.tex <==

% \begin{figure}[t!]
% \begin{center}
% \includegraphics[width=0.6\linewidth]{figures/inf_ver2.png}
% \includegraphics[width=0.3\linewidth]{figures/model_consensus.png}
% \caption{\textbf{ Influence of a word in a caption.} The darker the red color of a word, the greater its influence.
% For each caption, the noun with the highest EI score is underlined in red, and the noun with the lowest EI score is  underlined in gray.
% We can observe that some semantically important nouns such as `man' and `bathroom' have low EI scores, which can make a model not robust. 
% }
% \label{fig:inf_example}
% \end{center}
% \end{figure}

% \begin{figure*}[t!]
% \hspace{2mm}
% \begin{minipage}{0.5\linewidth}
% \centering
%   \includegraphics[width=0.9\linewidth]{figures/inf_ver2.png}
%   \caption{\textbf{Influence of a word in a caption.}}\label{fig:inf_example}
% \end{minipage}
% \hspace{5mm}
% \begin{minipage}{0.3\linewidth}
% \centering
%   \includegraphics[width=0.8\linewidth]{figures/model_consensus.png}
%   \caption{\textbf{Model Consensus.}}\label{fig:model_con∂sensus}
% \end{minipage}
% \vspace*{-5mm}
% \end{figure*}

\begin{figure}[h]
\centering
  \includegraphics[width=0.5\linewidth]{figures/inf_ver2.png}
  \caption{\textbf{Influence of a word in a caption.} The red color indicates higher influence.}\label{fig:inf_example}
  \vspace{-2mm}
\end{figure}



==> tables/vc-sc-i2t-table.tex <==
\begin{table*}[t]
\caption{\textbf{Improvement using Semantic and Visual Contrastive losses (BLIP ViT-B).}
We can observe improvement in robustness with the proposed SC \& VC losses. 
}
\label{table:vcsc-blip-i2t}
\centering
%\small
\resizebox{1\linewidth}{!}
{
\begin{tabular}{lccclccclccclccc}
\toprule
                         & \multicolumn{3}{c}{Rand-voca}           &                      & \multicolumn{3}{c}{Same-concept}        &                      & \multicolumn{3}{c}{Diff-concept}          &                      & \multicolumn{3}{c}{Danger}                \\ \cline{2-4} \cline{6-8} \cline{10-12} \cline{14-16} 
                         & R@1         & drop rate     & RSMS      &                      & R@1         & drop rate     & RSMS      &                      & R@1         & drop rate      & RSMS       &                      & R@1         & drop rate      & RSMS       \\ \hline
\multicolumn{16}{l}{\textbf{Image-to-Text Retrieval}}                                                                                                                                                                                                                              \\
BLIP ViT-B               & 64.50       & 21.25         & 23.72     & \multicolumn{1}{c}{} & 68.74       & 16.07         & 18.74     & \multicolumn{1}{c}{} & 69.20       & 15.51          & 17.36      & \multicolumn{1}{c}{} & 67.81       & 17.21          & 18.92      \\
\hspace{1mm}+SC Loss                & 70.16       & 14.34         & 13.07     & \multicolumn{1}{c}{} & 67.06       & 18.12         & 18.16     & \multicolumn{1}{c}{} & 69.78       & 14.79          & 14.37      & \multicolumn{1}{c}{} & 70.47       & 13.32          & 15.11      \\
\hspace{1mm}+SC\&VC Loss            & 71.20       & 13.06         & 13.94     & \multicolumn{1}{c}{} & 68.82       & 15.97         & 17.82     & \multicolumn{1}{c}{} & 71.93       & 12.17          & 13.67      & \multicolumn{1}{c}{} & 71.07       & 10.83          & 13.07      \\
VSE$\infty$(BUTD Region) & 31.71       & 45.34         & 47.99     & \multicolumn{1}{c}{} & 39.79       & 31.42         & 35.12     & \multicolumn{1}{c}{} & 36.91       & 36.38          & 39.86      & \multicolumn{1}{c}{} & 37.66       & 35.09          & 37.38      \\
\hspace{1mm}+SC Loss                & 37.24       & 35.82         & 39.46     & \multicolumn{1}{c}{} & 43.58       & 24.89         & 29.26     & \multicolumn{1}{c}{} & 42.95       & 25.97          & 30.13      & \multicolumn{1}{c}{} & 44.45       & 23.39          & 25.97      \\ \hline
                         & \multicolumn{3}{c}{Mix ($\lambda=0.9$)} &                      & \multicolumn{3}{c}{Mix ($\lambda=0.8$)} &                      & \multicolumn{3}{c}{Patch ($\lambda=0.9$)} &                      & \multicolumn{3}{c}{Patch ($\lambda=0.8$)} \\ \cline{2-4} \cline{6-8} \cline{10-12} \cline{14-16} 
                         & R@1         & drop rate     & RSMS      &                      & R@1         & drop rate     & RSMS      &                      & R@1         & drop rate      & RSMS       &                      & R@1         & drop rate      & RSMS       \\ \hline
\multicolumn{16}{l}{\textbf{Text-to-Image Retrieval}}                                                                                                                                                                                                                              \\
BLIP ViT-B               & 40.71       & 36.70         & 39.93     &                      & 46.97       & 26.96         & 30.84     &                      & 48.40       & 24.74          & 42.57      &                      & 52.61       & 18.19          & 21.45      \\
 + SC\&VC Loss            & 53.59       & 16.67         & 11.39     &                      & 57.05       & 12.10         & 5.15      &                      & 57.06       & 11.27          & 5.08       &                      & 57.41       & 10.73          & 4.45       \\ \bottomrule
\end{tabular}
\vspace*{-5mm}
}
\end{table*}
